Constraining A String Gauge Field by Galaxy Rotation Curves and Perihelion Precession of Planets

We discuss a cosmological model in which the string gauge field coupled universally to matter gives rise to an extra centripetal force and will have observable signatures on cosmological and astronomical observations. Several tests are performed using data including galaxy rotation curves of 22 spiral galaxies of varied luminosities and sizes, and perihelion precessions of planets in the solar system. The rotation curves of the same group of galaxies are independently fit using a dark matter model with the generalized Navarro--Frenk--White (NFW) profile and the string model. A Remarkable fit of galaxy rotation curves is achieved using the one-parameter string model as compared to the three-parameter dark matter model with the NFW profile. The average $\chi^2$ value of the NFW fit is 9\% better than that of the string model at a price of two more free parameters. Furthermore, from the string model, we can give a dynamical explanation for the phenomenological Tully-Fisher relation. We are able to derive a relation between field strength, galaxy size and luminosity, which can be verified with data from the 22 galaxies. To further test the hypothesis of the universal existence of the string gauge field, we apply our string model to the solar system. Constraint on the magnitude of the string field in the solar system is deduced from the current ranges for any anomalous perihelion precession of planets allowed by the latest observations. The field distribution resembles a dipole field originating from the Sun. The string field strength deduced from the solar system observations is of a similar magnitude as the field strength needed to sustain the rotational speed of the Sun inside the Milky Way. This hypothesis can be tested further by future observations with higher precision.

==> DM-string_fit_mass_summaries_tables.tex <==
%\fig{DM_mass_summary}{%
%Summary of stellar mass and mass of dark matter halos computed from the best fit values, as well as mass to light ratios of the 22 galaxies in the dark matter model.  The mass is in units of $M_{sun}$. Mass to light ratio is relative to the mass of light ratio of the Sun.%
%}{0.9}
%
\begin{table}
\begin{center}
  \begin{tabular}{|l|c|c|c|c|c|c|}
  \tableline
galaxy&	B-magnitude&	 M$^{*}$&	DM+M*&	 M/L&	log(M/L)&	M*/DM\\\tableline \tableline
m81dwb&	-12.5&	4.07E+06&	7.89E+08&	50.72&	1.71&		3.12\% \\\tableline
ngc0628&	-20.60&	2.74E+10&	3.34E+12&	123.36&	2.09&		1.00\% \\\tableline
ngc0925&	-20.05&	2.08E+08&	2.26E+12&	138.71&	2.14&		0.16\% \\\tableline
ngc2403&	-19.56&	1.55E+08&	1.70E+12&	164.12&	2.22&		0.07\% \\\tableline
ngc2976&	-18.12&	7.79E+09&	4.79E+12&	1738.70&	3.24&		0.14\% \\\tableline
ngc3031&	-21.54&	2.17E+10&	3.83E+12&	59.63&	1.78&		3.42\% \\\tableline
ngc3184&	-19.88&	2.39E+10&	2.46E+12&	176.74&	2.25&		3.16\% \\\tableline
ngc3198&	-20.44&	1.88E+07&	4.71E+11&	20.18&	1.30&		8.90\% \\\tableline
ngc3521&	-21.08&	1.54E+08&	8.70E+11&	20.68&	1.32&		4.83\% \\\tableline
ngc3621&	-20.51&	1.41E+11&	1.94E+11&	7.81&	0.89&		2.37\% \\\tableline
ngc3938&	-20.01&	5.35E+09&	8.86E+11&	56.45&	1.75&		1.70\% \\\tableline
ngc4236&	-18.10&	2.51E+10&	7.30E+10&	27.01&	1.43&		0.61\% \\\tableline
ngc4321&	-22.06&	5.11E+08&	2.20E+12&	21.25&	1.33&		2.58\% \\\tableline
ngc4536&	-21.79&	4.96E+07&	6.24E+11&	7.71&	0.89&		11.57\% \\\tableline
ngc4569&	-21.10&	2.67E+08&	2.09E+12&	48.82&	1.69&		0.32\% \\\tableline
ngc4579&	-21.68&	2.88E+11&	8.96E+11&	12.26&	1.09&		7.57\% \\\tableline
ngc4625&	-17.63&	6.45E+08&	2.95E+12&	1683.06&	3.23&		0.06\% \\\tableline
ngc4725&	-21.76&	7.00E+09&	6.76E+12&	85.89&	1.93&		3.34\% \\\tableline
ngc5055&	-21.20&	1.13E+10&	5.00E+11&	10.64&	1.03&		8.81\%\\\tableline
ngc5194&	-20.51&	2.25E+09&	8.27E+10&	3.32&	0.52&		8.44\%\\\tableline
ngc6946&	-20.89&	2.19E+10&	7.09E+13&	2006.87&	3.30&		0.02\%\\\tableline
ngc7331&	-21.58&	8.09E+07&	1.33E+12&	19.92&	1.30&		3.24\%\\\tableline
\end{tabular}
    \caption{%
Summary of stellar mass and mass of dark matter halos computed from the best fit values, as well as mass to light ratios of the 22 galaxies in the dark matter model.  The mass is in units of $M_{sun}$. Mass to light ratio is relative to the mass of light ratio of the Sun.}
\label{DM_mass_summary}
\end{center}
\end{table}




%\fig{string_mass_summary}{%
%Summary of stellar mass as well as mass to light ratios as computed from the best fit values in string model. The mass of the galaxies is in units of $M_{sun}$. Mass to light ratio is relative to the mass of light ratio of the Sun.%
%}{0.8}
\begin{table}
\begin{center}
  \begin{tabular}{|l|c|c|c|c|}
  \tableline
galaxy&	B-magnitude&	$\Omega$(Hz$\cdot$km/kpc)&	total mass($M_sun$)&	 mass/light
 \\\tableline \tableline
m81dwb&	-12.5&		1.1193&	2.46E+07&	1.5814\\\tableline
ngc0628&	-20.60&	8.8716&	3.35E+10&	1.2388\\\tableline
ngc0925	&-20.05&	5.08&	3.68E+09&	0.2261\\\tableline
ngc2403	&-19.56&	13.4183&	1.12E+09&	0.1076\\\tableline
ngc2976	&-18.12&	0.10&	6.76E+09&	2.4549\\\tableline
ngc3031	&-21.54&	2.00&	1.31E+11&	2.0420\\\tableline
ngc3184	&-19.88&	0.6553&	7.77E+10&	5.5805\\\tableline
ngc3198	&-20.44&	1.9685&	4.19E+10&	1.7963\\\tableline
ngc3521	&-21.08&	6.0462&	4.20E+10&	0.9990\\\tableline
ngc3621	&-20.51&	10.3377&	4.60E+09&	0.1848\\\tableline
ngc3938	&-20.01&	9.7216&	1.50E+10&	0.9577\\\tableline
ngc4236	&-18.10&	10.3577&	4.42E+08&	0.1636\\\tableline
ngc4321	&-22.06&	5.2077&	5.70E+10&	0.5492\\\tableline
ngc4536	&-21.79&	1.4650&	7.22E+10&	0.8919\\\tableline
ngc4569	&-21.10&	16.37&	6.75E+09&	0.1575\\\tableline
ngc4579	&-21.68&	7.39&	6.79E+10&	0.9286\\\tableline
ngc4625	&-17.63&	0.10&	1.68E+09&	0.9565\\\tableline
ngc4725	&-21.76&	1.3785&	2.26E+11&	2.8680\\\tableline
ngc5055	&-21.20&	4.0642&	4.40E+10&	0.9373\\\tableline
ngc5194	&-20.51&	3.1862&	6.98E+09&	0.2803\\\tableline
ngc6946	&-20.89&	7.4403&	1.43E+10&	0.4037\\\tableline
ngc7331	&-21.58&	8.4646&	4.30E+10&	0.6446\\ \tableline
\end{tabular}
    \caption{%
Summary of stellar mass as well as mass to light ratios as computed from the best fit values in string model. The mass of the galaxies is in units of $M_{sun}$. Mass to light ratio is relative to the mass of light ratio of the Sun.}
\label{string_mass_summary}
\end{center}
\end{table}




==> best_fit_DM_table.tex <==
%%   \fig{best_fit_DM}
%%   {best_fit_DM}
\begin{table}
\begin{center}
  \begin{tabular}{|l|c|c|c|c|c|c|}
  \tableline
galaxy& liklihood&	$R_{d}(kpc)$&	$\frac{r_{s}}{R_{d}}$& $\alpha$ &$\rho$& $\sigma$ \\
\tableline \tableline
m81dwb&	0.158	&0.24&	8.2&	1.54	&613	&19.2\\ \tableline
ngc0628	&4.398	&1.88&	9.9	&0.75	&8409&	98.4 \\ \tableline
ngc0925	&2.392	&0.79&	27.6&	0.22&	859&	56.6 \\ \tableline
ngc2403	&4.467	&0.75&	21.1&	0.76&	744&	84.6\\ \tableline 
ngc2976	&0.504	&2.52&	18.3&	0.38&	998&	16.8\\ \tableline
ngc3031	&5.614	&3.99&	5.9	& 0.96	&705	&57.7\\ \tableline
ngc3184	&0.573	&3.97&	6.1	&0.58	&784	&42.1\\ \tableline
ngc3198	&0.441	&0.51&	18.2&	1.09&	291	&99.95\\ \tableline
ngc3521	&0.167	&0.57&	18.8&	1.56&	&1738&	99.5\\ \tableline
ngc3621	&0.125	&6.85&	1.8	&1.80	&903	&5.6\\ \tableline
ngc3938	&0.905	&2.45&	5.5	&1.33	&747	&60.6\\ \tableline
ngc4236	&1.180	&4.40&	6.5	&0.83	&603	&1.4\\ \tableline
ngc4321	&0.956	&0.87&	19.6&	1.02&	1581&	80.5\\ \tableline
ngc4536	&0.598	&0.99&	10.7&	0.86&	105	&97.2\\ \tableline
ngc4569	&0.651	&0.74&	18.1&	0.95&	1350&	145.4\\ \tableline
ngc4579	&0.719	&7.90&	4.3	&1.80	&1200	&3.4\\ \tableline
ngc4625	&0.874	&1.91&	14.1&	0.20&	&191&	42.6\\ \tableline
ngc4725	&0.481	&4.00&	7.5	&0.77	&225	&53.9\\ \tableline
ngc5055	&1.133	&2.25&	4.5	&1.66	&2044	&67.0\\ \tableline
ngc5194	&0.442	&1.45&	4.4	&1.50	&1518	&49.9\\ \tableline
ngc6946	&5.670	&2.62&	29.4&	0.27&	2491&	42.6\\ \tableline
ngc7331	&0.839	&0.50&	19.6&	1.32&	1325&	197.7\\ \tableline
  \end{tabular}
  \caption{%
Best fit values for the five free parameters in the Dark Matter model with generalized NFW profile.}
\label{best_fit_DM}
\end{center}
\end{table}

==> best_fit_string_table.tex <==
%%   \fig{best_fit_string}
%%   {Best fit values for the three free parameters in the string model.}
\begin{table}
\begin{center}
  \begin{tabular}{|l|c|c|c|c|}
  \tableline
galaxy&	likelihood&	$\Omega(Hz$\cdot$km/kpc)& $\rho$&	$R_d$(kpc) \\\tableline \tableline
m81dwb&	0.125&	1.119&	15919&	0.15\\ \tableline
ngc0628&	4.347&	8.872&	11738&	1.80\\ \tableline
ngc0925&	2.452&	5.077&	500&	2.47\\ \tableline
ngc2403&	4.247&  13.418&	16497&	0.52\\ \tableline
ngc2976&	0.400&	0.100&	2135&	1.87\\ \tableline
ngc3031&	5.698&	2.000&	3187&	4.39\\ \tableline
ngc3184&	0.574&	0.655&	1552&	4.69\\ \tableline
ngc3198&	0.275&	1.968&	1971&	3.52\\ \tableline
ngc3521&	0.588&	6.046&	26678&	1.48\\ \tableline
ngc3621&	0.366&	10.338&	7413&	1.08\\ \tableline
ngc3938&	1.030&	9.722&	16199&	1.24\\ \tableline
ngc4236&	0.325&	10.358&	110&	2.02\\ \tableline
ngc4321&	2.070&	5.208&	3752&	3.15\\ \tableline
ngc4536&	0.739&	1.465&	734& 	5.87\\ \tableline
ngc4569&	0.662&	16.370&	12262&	1.04\\ \tableline
ngc4579&	0.688&	7.385&	5164&	3.00\\ \tableline
ngc4625&	0.548&	0.100&	1140&	1.45\\ \tableline
ngc4725&	0.268&	1.378&	1523&	6.73\\ \tableline
ngc5055&	3.521&	4.064&	24581&	1.54\\ \tableline
ngc5194&	0.807&	3.186&	10718&	1.10\\ \tableline
ngc6946&	6.035&	7.440&	4980&	1.80\\ \tableline
ngc7331&	0.522&	8.465&	18613&	1.68\\ \tableline
\end{tabular}
    \caption{%
Best fit values for the three free parameters in the string model.}
\label{best_fit_string}
\end{center}
\end{table}

==> galaxy_measurement_table.tex <==
%\fig{galaxy_measurement}
%{%
%Relevant galaxy observation data for determining luminosity and distance.%
%}{0.7}
\begin{table}
\begin{center}
  \begin{tabular}{|l|c|c|c|}
  \tableline
galaxy&	B-magnitude&	mucin&	Distance \\\tableline \tableline
m81dwb&	-12.5&	N/A& 	3.5 \\ \tableline
ngc0628&	-20.60&	29.95&	9.77\\ \tableline
ngc0925&	-20.05&	29.85&	9.33\\ \tableline
ngc2403&	-19.56&	27.68&	3.44\\ \tableline
ngc2976&	-18.12&	28.10&	4.17\\ \tableline
ngc3031&	-21.54&	28.57&	5.18\\ \tableline
ngc3184&	-19.88&	30.20&	10.96\\ \tableline
ngc3198&	-20.44&	30.42&	12.13\\ \tableline
ngc3521&	-21.08&	30.29&	11.43\\ \tableline
ngc3621&	-20.51&	29.58&	8.24\\ \tableline
ngc3938&	-20.01&	30.81&	14.52\\ \tableline
ngc4236&	-18.10&	27.08&	2.61\\ \tableline
ngc4321&	-22.06&	31.90&	23.99\\ \tableline
ngc4536&	-21.79&	32.11&	26.42\\ \tableline
ngc4569&	-21.10&	30.52&	12.71\\ \tableline
ngc4579&	-21.68&	31.80&	22.91\\ \tableline
ngc4625&	-17.63&	30.35&	11.75\\ \tableline
ngc4725&	-21.76&	31.45&	19.50\\ \tableline
ngc5055&	-21.20&	30.09&	10.42\\ \tableline
ngc5194&	-20.51&	30.01&	10.05\\ \tableline
ngc6946&	-20.89&	29.12&	6.67\\ \tableline
ngc7331&	-21.58&	30.75&	14.13\\ \tableline
\end{tabular}
    \caption{%
Relevant galaxy observation data for determining luminosity and distance.}
\label{galaxy_measurement}
\end{center}
\end{table}

==> table_RC.tex <==
\begin{table}
\begin{center}
  \begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \tableline
galaxy &	m81dwb & ngc0628 & ngc0925 &	ngc2403 &	ngc2976 &	ngc3031 &	ngc3184 &	ngc3198 & ngc3521 & ngc3621 &ngc3938 &	ngc4236 &	ngc4321 &	ngc4536 &	ngc4569 &	ngc4579 &	ngc4625 &	ngc4725 &	ngc5055 & ngc5194 &	ngc6946 &	ngc7331 \\
\tableline

\tableline 
  \end{tabular}
  \caption{%
{Best fit values for the three free parameters in the string model.}
}
\label{best_fit_string}
\end{center}
\end{table}
